Consequences of parameterization choice on eclipsing binary light curve solutions

Eclipsing Binaries (EBs) are known to be the source of most accurate stellar parameters, which are important for testing theories of stellar evolution. With improved quality and quantity of observations using space telescopes like {\it TESS}, there is an urgent need for accuracy in modeling to obtain precise parameters. We use the soon to be released \texttt{PHOEBE 2.3} EB modeling package to test the robustness and accuracy of parameters and their dependency on choice of parameters for optimization.

==> 1_-_Introduction.tex <==
\section{Introduction} \label{intro}\setlength{\parindent}{0pt}
\begin{comment}
Eclipsing Binaries (EBs) are known to be the source of most accurate stellar parameters, which are important for testing theories of stellar evolution. Precise photometric observations using space-based telescopes like the Transiting Exoplanet Survey Satellite \citep[\TESS;][]{tess2014} reveal the need for accurate modeling of the EBs to obtain precise stellar parameters. 

Moreover, it is possible to observe and study astronomical phenomena in details never seen before (e.g. reflection from the companion, lensing, or Doppler beaming).
\end{comment}

It is well known that EBs provide highly accurate observations of stellar parameters, which is important for testing theories of star evolution. Thanks to the increasingly more precise photometry of the past and recent space missions (e.g. \textit{Kepler} \citep{borucki2016} and the Transiting Exoplanet Survey Satellite \citep[\TESS;][]{tess2014}), it is now possible to observe and study EBs in details never seen before (e.g. reflection from the companion, lensing, or Doppler beaming). To understand the observations, one needs to employ models capable of making predictions with sufficient precision, so that it is possible to compare the observations with predicted theoretical values. A popular example of such software is \textsc{PHOEBE} \citep{phoebeprsa, phoebehov, phoebejones}, a robust Python package for modeling of EB systems. The latest release provides users with control over a large number of orbital and physical parameters, which allows them to generate synthetic light curves and radial velocities of the binary system. One can also take advantage of various built-in or imported solvers (e.g. \textsc{emcee}) and optimizers (e.g. Nelder-Mead) to solve the inverse problem---for a comprehensive introduction to the inverse problem using PHOEBE see \cite{kylephoebe2.3}.

For the purpose of this paper, we use the soon to be released version 2.3 of \textsc{PHOEBE} to try and reproduce the results from the article by \cite{maxted2020}, which examines a number of various methods to accurately estimate the masses and radii for the stars in the binary system AI Phoenicis (AI Phe). This system, which contains two well-separated, sharp-lined stars of comparable luminosity, was first identified as an EB by \cite{strohm}. It is an excellent target for model testing as it is relatively bright ($V = 8.6$ mag), has a long orbital period ($P\approx24.59$ days), and does not show any distinct spots nor flares associated with increased magnetic activity of the components \citep[e.g.,][]{kkent2016, maxted2020}.

To compare the results by \citet{maxted2020}, we first carried out a number of runs with varying underlying physical models, free parameters, and their initial values (see Section~\ref{dataset}). This further motivated us to design a controlled experiment in order to systematically analyze the effect of parameterization choice on the final light curve resulting from the model (Section \ref{contrexp}). Finally, in Section~\ref{discussion} we compare our results from the controlled experiment with the \citet{maxted2020} values, and we discuss our findings regarding the precision of the employed model.




==> 2_-_Used_dataset_and_modeling_set-up.tex <==
\section{Observations and Modeling Set-up} \label{dataset}
The photometric data of AI Phe used in the subsequent analyses were obtained under the \TESS{} Guest Investigator Program (G011130, P.I. Maxted; G011083, P.I. Hełminiak; G011154, P.I. Prša) during Sector 2 of the \TESS{} mission observed in the 2-min cadence mode (TIC 102069549). The Sector was observed for 27 days from $2458354.113259$ BJD to $2458381.517643$ BJD (covering both the primary and secondary eclipse), and the data were reduced by the \TESS{} data processing pipeline developed by the Science Processing Operations Center \citep[SPOC;][]{jenkins2016}. In our analyses, we used the Pre-search Data Conditioning Simple Aperture Photometry (\pdcsap) light curve, which was additionally detrended by fitting a chain of $5^{th}$ order Legendre polynomials \citep[][Section 2.6]{maxted2020}.

To get a sense of the effect of parameterization on the resulting values, we independently solved the inverse problem for AI Phe by using a separate model with its own set of free parameters and approximation of physical phenomena (e.g. limb-darkening law, reflection, etc.). Following the approach from \cite{maxted2020}, we initialized the parameters of the models with their estimates from \citet{kkent2016}, which are summarized in Table \ref{kentdata2}.

\begin{table}[h!] 
\caption{A list of the parameters of the binary system AI Phe that were adopted from \cite{kkent2016}.}
\label{kentdata2}
\centering
\begin{tabular}{ll}
\hline
\hline
Parameters  & Values\\
\hline
$P$ (days) & 24.592483  \\
$q$ & 1.0417   \\
$e$ & 0.1821  \\
$\omega(^{o}$ )& 110.73 \\
$i(^{o}$ ) & 88.502 \\
$M_{1}$ (\(M_\odot\)) & 1.1973 \\
$M_{2}$ (\(M_\odot\))& 1.2473 \\
$R_{1}$ (\(R_\odot\)) & 1.835 \\
$R_{2}$ (\(R_\odot\))&  2.912 \\
$T_{1}$ (K) & 6310 \\
$T_{2}$ (K)&  5237.3 \\
\hline
\hline
\end{tabular}
\end{table}

The initialized free parameters were used as input to the Nelder-Mead algorithm \citep{nmead} in order to refine the estimates. These estimates then served as a starting point for initial distributions (either Gaussian or uniform) of the free parameters entering the Markov Chain Monte Carlo (MCMC) algorithm implemented in the \textsc{emcee} solver \citep{emcee}, which we used to obtain posterior distributions of the relevant parameters. Furthermore, we used the following software: \textsc{Python} \citep{python}, and the \textsc{Python} libraries \textsc{Matplotlib} \citep{matplotlib} and \textsc{numpy} \citep{numpy}. 

Unfortunately, the individual runs did not yield satisfactory results as the obtained values showed a wide spread. Due to the different choices of parameterization and the large numbers of parameters, it was not possible to associate the observed variation with a specific parameter or a set of parameters. Therefore, we decided to design a controlled experiment, in which we defined a ``nominal" run and then we examined the effect of altering the parameters one at a time. For more information see the following section.



==> 3_-_Controlled_experiment.tex <==
\section{Controlled Experiment} \label{contrexp}
The ``nominal" run (which we shall denote ``Run A") served as a benchmark for all the other runs (``B" through ``K"), which we systematically varied from Run A in a controlled fashion---that is, for each run, we altered one aspect of the ``nominal" set-up and kept the rest unchanged. For the definitions of Runs B--K, see Table \ref{runstab}.

\begin{table}[h!] 
\caption{A list of the individual runs and their differences from the ``nominal" run.}
\label{runstab}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ll}
\hline
\hline
Run  & Description\\
\hline
A & The ``nominal" run  \\
B & Logarithmic limb darkening law\\
C & Sample/interpolate in phase-space \\
D & Marginalization over albedos \\
E & Marginalization over gravity darkening parameters\\
F %E2%
& Marginalization over gravity darkening parameters from \\ &  \cite{gravdcoeff} \\
G %F 
& Marginalization over noise nuissance parameter\\
H %G
& Marginalization over parameters $q$ and $a$ using radial velocities \\ & posteriors from \cite{rvdata} on $q$ and $a\sin{i}$\\
I & Meshes on binary surfaces to estimate $L_\mathrm{pb}$\\
J & \TESS{} light curve without detrending (PDCSAP)\\
K %L
&  Masking the out-of-eclipse points \\
\hline
\hline
\end{tabular}}
\end{table}

Run A uses the binary star model \textsc{ellc} \citep[for more information see][]{ellc} with the quadratic limb-darkening law in the ``lookup" mode (automatic querying of coefficients from tables based on mean stellar values), and uses the Stefan-Boltzmann approximation in the determination of the passband luminosity, $L_\mathrm{pb}$, which is needed to scale the fluxes and estimate the surface-brightness ratio. Similar to our initial test runs, we initialized the parameters with values from \cite{kkent2016}, and then used the Nelder-Mead algorithm to refine the estimates. After that, we used the \textsc{emcee} solver to sample over the radii, $R_1$ and $R_2$, (for the primary and secondary component), the eccentricity, $e$, along with the argument of pericenter, $\omega_{0}$, (parameterized as $e \sin{\omega_{0}}$ and $e \cos{\omega_{0}}$), the time of the primary eclipse, $T_{0}$, the third light, $l_{3}$, $L_\mathrm{pb}$, the ratio of the effective temperature of the secondary and primary component, $T_\mathrm{secondary}/T_\mathrm{primary}$, and the orbital inclination, $i$, to get an estimate for their uncertainties. We present the obtained results in Fig. \ref{fig:comparison}

\begin{figure}[!htb]
\begin{subfigure}{0.5\textwidth}
\leftline{
\includegraphics[width=\linewidth]{final/figures/compare_maxted_first.eps}
}
\label{fig:a}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\leftline{
\includegraphics[width=\linewidth]{final/figures/compare_maxted_second.eps}
}
\label{fig:b}
\end{subfigure}

\vspace{0.2cm}
\begin{subfigure}{0.5\textwidth}
\leftline{
\includegraphics[width=\linewidth]{final/figures/compare_maxted_third.eps}
}
\label{fig:c}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\leftline{
\includegraphics[width=\linewidth]{final/figures/compare_maxted_fourth.eps}
}
\label{fig:d}
\end{subfigure}

\vspace{0.2cm}
\begin{subfigure}{0.5\textwidth}
\leftline{
\includegraphics[width=\linewidth]{final/figures/compare_maxted_fifth.eps}
}
\label{fig:e}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\leftline{
\includegraphics[width=\linewidth]{final/figures/compare_maxted_sixth.eps}
}
\label{fig:f}
\end{subfigure}
\caption{A comparison between the parameters resulting from Runs A--K and those obtained by \citet{maxted2020}. The filled rectangle represents the 1-$\sigma$ spread around the average of the runs from the Maxted et al. paper (see Table \ref{tab3}), while the dotted box shows the same for our controlled runs. The inner box in the $l_{3}$ vs $i$ plot represents a zoomed-in view on the  parameter distribution.}
\label{fig:comparison}
\end{figure}

\begin{comment}
Therefore, we created a ``nominal setup" as a reference case (Run A) and varied some parameters and their initializations. The nominal setup uses the \textsc{ellc} binary star model from \citet{ellc} with the quadratic limb-darkening law in ``lookup" mode (automatic query of coefficients from tables), the passband luminosity ($L_\mathrm{pb}$; used to scale the fluxes and estimate the surface brightness ratio) is determined using a `Stefan-Boltzmann' approximation \citep{kylephoebe2.3}, and the parameters are initialized with the values from \cite{kkent2016}. The parameters were first optimized using Nelder-Mead and then the radii ($R_\mathrm{equiv}$; both primary and secondary), the eccentricity along with argument of pericentre (parameterized via $e \sin{\omega_{0}}$ and $e \cos{\omega_{0}}$), the time of primary eclipse ($T_{0}$), the third light ($l_{3}$), $L_\mathrm{pb}$, the ratio of effective temperatures ($T_\mathrm{secondary}/T_\mathrm{primary}$), and the orbital inclination of the binary ($i$) were sampled using \textsc{emcee} to estimate uncertainties (see Table.\ref{tab4}). Details of the individual runs are given in Table \ref{runstab}. It summarizes the differences of each run in regard to the nominal Run A. %The posterior distributions for some parameters are shown in Fig.~\ref{fig:comparison}. 
%\begin{itemize}
%    \item \textbf{Run A:} The ``Nominal Run" is initialized with the parameter values from \cite{kkent2016} and optimized with Nelder Mead followed by MCMC sampling to obtain the posteriors. We used the \textit{ellc} \citep{ellc} binary star model, which is an available fitting model in \phoebe{}. The parameters that were optimized includes $R_{equivalent} $ (both primary and secondary), $esin\omega_{0}$, $ecos\omega_{0}$, $a$, $l_{3}$, $L_{pb}$, ratio of $T_{eff}$ and $i$. The successive runs all have the same parameters and models used, unless stated otherwise.
%    \item \textbf{Run B:} This run used a logarithmic limb darkening law rather than the quadratic limb darkening law as in the ``nominal run". 
%    \item \textbf{Run C:} This run was computed by using the times as computed before while defining the data-set (equally spaced points between 0 and 1). The ``nominal run" was calculated using times from the data-set itself. 
%    \item \textbf{Run D:} Additional parameters for irradiation of both the primary and secondary components was added to be marginalized using MCMC along with the parameters of the% Run-A.
%    \item \textbf{Run E:} Parameters for gravity darkening for both the components were added to be marginalized along with the Run-A parameters. 
%    \item \textbf{Run E2:} The values for gravity darkening were defined in this run. The values of the parameters were taken from \cite{gravdcoeff} and fixed to be 0.26  and 0.5 respectively for the primary and secondary components, similar to \cite{kkent2016}.
%    \item \textbf{Run F:} \phoebe{} provides an option to correct for observation uncertainty underestimation. In this run, we allow for estimation and correction of this underestimation.
 %   \item \textbf{Run G:} This run involves an additional data-set along with the light-curve in Run A. We use radial velocity observations from \cite{rvdata}. Initially, we optimize and marginalize over parameters $v_{\gamma}$, $q$ and $asini$. We then adopt values and distributions of $q$ and $asini$ as priors to fit the light-curve with rest of the parameters same as Run A.
 %   \item \textbf{Run H:} We switch to the PHOEBE model from \textit{ellc}t for this run. Additionally, we change the limb darkening mode to `interpolation' which was not available for the \textit{ellc} backend. 
  %  \item \textbf{Run I:} For this run, we change the $pblum\_mode$ to \textit{phoebe}. This controls the scaling of the model generated. 
  %  \item \textbf{Run J:} We used an alternatively detrended \tess{} light curves for this run, keeping all the parameters same as Run A.
  %  \item \textbf{Run K:} While all the runs had passbands defined as `TESS:T' while loading data-sets to the model, we changed the passband in this run to `Johnson:V'. This was done in order to check if computing parameters using wrong passband can have drastic effects.
  %  \item \textbf{Run JK:} For this run, we combined the changes in runs J and K while keeping everything the same as Run A.
  %  \item \textbf{Run L:} For this run, we masked the data-set for light-curves so as only to fit the points in the eclipses only. 
%\end{itemize}



\begin{table}[h!] 
\caption{The individual runs and their differences to the ``Nominal Run".}
\label{runstab}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ll}
\hline
\hline
Run  & Description\\
\hline
A & The ``Nominal Run"  \\
B & Logarithmic limb darkening law\\
C & Sample/interpolate in phase-space \\
D & Marginalization over albedos \\
E & Marginalization over gravity darkening parameters\\
F %E2%
& Marginalization over gravity darkening parameters from \\ &  \cite{gravdcoeff} \\
G %F 
& Marginalization over noise nuissance parameter\\
H %G
& Marginalization over parameters $q$ and $a$ using radial velocities \\ & posteriors from \cite{rvdata} on $q$ and $a\sin{i}$\\
I & Meshes on binary surfaces to estimate $L_\mathrm{pb}$\\
J & \TESS{} light curve without detrending (PDCSAP)\\
K %L
&  Masking the out-of-eclipse points \\
\hline
\hline
\end{tabular}}
\end{table}

\end{comment}
%\begin{table}[t]

%\small
%\begin{center}
%\caption{The different runs with different variations in parameters, models or values of parameters. The rest of the details about the runs are similar to Run A.}
%\label{runstab}
%\adjustbox{max width=\linewidth}{
%\begin{tabular}{ll}
%\hline
%\textbf{Run}  & \textbf{Description}\\
%\hline
%\hline 
%A &  The ``Nominal Run".  \\
%\hline
%B &   Logarithmic limb darkening law rather than the quadratic limb darkening law.   \\
%\hline
%C &   Run using computer generated times (equally spaced points between 0 and 1).  \\
%\hline
%D &   Additional irradiation parameters of both the components were marginalized. \\
%\hline
%E &   Additional gravity darkening parameters for both the components were marginalized. \\
%\hline
%E2 &   The value of gravity darkening parameters were taken from \cite{gravdcoeff}. \\
%\hline
%F &   We allow for estimation and correction of underestimation of the data uncertainty. \\
%\hline
% &   We marginalize over parameters $v_{\gamma}$, $q$ and $asini$ using radial velocities from \\
% G &  \cite{rvdata}. We then adopt distributions of $q$ and $asini$ as priors to fit  \\
 % & the light curve. \\
% \hline
%H &   We switch to the PHOEBE model from \textit{ellc} and change the limb darkening mode to  \\
%& `interpolation'. \\ 
%\hline
%I &  We change the $pblum\_mode$ to \textit{phoebe} which controls the scaling of the generated model. \\
%\hline
%J &  We used an alternatively detrended \tess{} light curve.  \\
%\hline
%K &  We changed the passband in this run to `Johnson:V'. This was done in order to check if   \\
%& computing parameters using wrong passband can have drastic effects.\\
%\hline
%JK &   For this run, we combined the changes in runs J and K .\\
%\hline
%L &   We masked the data-set for light-curves so as only to fit the points in the eclipses only. \\
%\hline  
%\end{tabular}
%}
%\end{center}

%\end{table}


==> 4_-_Discussion_of_results.tex <==
\section{Discussion of Results} \label{discussion}
Analysis of Runs A--K shows a rather limited spread of the obtained values, with the individual parameters lying within each other's uncertainties (see Fig. \ref{fig:comparison}). Seeing that the parameters have a fairly small effect on the final results, this implies that the high variation of our initial runs was most likely not caused by any specific parameter but rather by a combined effect of various parameterization choices.  That said, it is still clear that the choices made in Table \ref{runstab} do influence the final results.

\textbf{} As for the results obtained by \citet{maxted2020}, Runs A and S by Maxted (see Table \ref{tab3}) are especially of interest to us as they use the binary star model \textsc{ellc} together with \textsc{emcee} optimization (our runs use a wrapper for mapping of \textsc{PHOEBE} parameterization onto \textsc{ellc}), and thus their outputs can be a benchmark for our results. Note that for the sake of simplicity, we shall mainly focus on our Run A---for the definitions of the other runs see Table \ref{runstab}. Moreover, Runs A and S by Maxted use essentially the same initial set-ups, therefore it suffices to examine only the former (which additionally corrects for instrumental systematic variations). To avoid confusion, we shall refer to Runs A and S by \citet{maxted2020} as ``Run M-A" and ``Run M-S" in the rest of the section.

In Table \ref{tab4}, we compare the free parameters entering the \textsc{emcee} algorithm in Run M-A and our Run A. Apart from working with mostly disjunct (but correlated) sets of free parameters, the two runs also differ in the limb-darkening law (power-2 for Run M-A and quadratic for Run A) and the treatment of the stellar masses. Run A adopts the values 1.1973 M$_{\odot}$ and 1.0417 from \cite{kkent2016} for the mass of the primary component and the ratio of the masses of the secondary and primary component, respectively. In addition, the stellar masses are held constant at the Kirkby-Kent values as they have minimal effect on the light curve. In contrast, Run M-A uses the \textsc{emcee} posterior distributions of the free parameters together with observed radial velocities of the binary system to get an estimate for the masses. Finally, both runs hold the semi-major axis constant, with Run M-A assuming the value of 47.868 R$_{\odot}$ and Run A keeping it equal to 47.941 R$_{\odot}$.

\begin{table}[h!] 
\caption{An overview of the various runs analysed in the paper by \cite{maxted2020}. The table was adopted from page 6 of the mentioned paper.}
\label{tab3}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{llllll<{\raggedleft}m{4cm}}
\hline
\hline
Run & Investigator & Model & Optimization & Limb-darkening & Detrending & Notes\\
\hline
A & Maxted & \textsc{ellc} & \textsc{emcee} & power-2 & \textsc{celerite} & \\
B & Helminiak & JKTEPOB & L-M & quadratic & sine+poly & Monte Carlo error estimated\\
C & Torres & EB & \textsc{emcee} & quadratic & spline & Quadratic l.d. coeffs. fixed\\
D & " & " & " & " & " & \\
E & Graczyk & WD2007 & L-M & logarithmic & -- & Fixed l.d. coefficients\\
F & Johnston & \textsc{phoebe 1.0} & \textsc{emcee} & square-root & -- & \\
G & Prša & \textsc{phoebe 2.1} & MCMC & grid & legendre & \\
H & Orosz & ELC & DE-MCMC & logarithmic & polynomial & \\
I & Orosz & " & " & square-root & " & \\
J & Orosz & " & " & quadratic & " & \\
K & Southworth & JKTEBOP & L-M & quadratic & polynomial & \\
L & Southworth & JKTEBOP & L-M & cubic & polynomial & \\
S & Maxted & \textsc{ellc} & \textsc{emcee} & power-2 & \textsc{celerite} & Same as Run A with SAP light curve\\
\hline
\hline
\end{tabular}}
\end{table}

\begin{comment}
\begin{table}[h!] 
\caption{A list of the free parameters entering the \textsc(emcee) algorithm in Runs M-A and A. To speed-up the execution of Run A, we first obtained initial estimates for the parameters $T_\mathrm{primary}/T_\mathrm{secondary}$, $i$, $e \sin{\omega}$, $e \cos{\omega}$, $R_1$, $R_2$ and $T_\mathrm{0}$ using the NM algorithm.} \label{tab2}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ll|ccc}
\hline
\hline
Parameter & Description & Run M-A & Run A\\
\hline
$e \cos{\omega}$ &  &  & \checkmark\\
$e \sin{\omega}$ &  &  & \checkmark\\
$f$ & Flux scaling factor & \checkmark & \\
$f_c$ & $\sqrt{e}\cos{\omega}$ & \checkmark & \\
$f_s$ & $\sqrt{e}\sin{\omega}$ & \checkmark & \\
$h_\text{1,F}, h_\text{2,F}$ & Parameters of the power-2 limb darkening law for star 1 & \checkmark & \\
$h_\text{1,K}, h_\text{2,K}$ & Parameters of the power-2 limb darkening law for star 2 & \checkmark & \\
$i$ & Orbital inclination & \checkmark & \checkmark\\
$k$ & Ratio of the radii & \checkmark & \\
$l_3$ & Third light & \checkmark & \checkmark\\
$pblum$ & Passband luminosity &  & \checkmark\\
$r_{sum}$ & Sum of the fractional radii & \checkmark & \\
$R_1$ & Radius of the primary star &  & \checkmark\\
$R_2$ & Radius of the secondary star &  & \checkmark\\
$\sigma_f$ & Standard error per observation & \checkmark & \\
$S_{\text{T}}$ & Surface brightness ratio averaged over the stellar disks in the TESS band & \checkmark & \\
$\text{T}_\text{0}$ & Time of primary eclipse & \checkmark & \checkmark\\
$T_\text{primary}/T_\text{secondary}$ & Ratio of the effective temperatures &  & \checkmark\\
\hline
\hline
\end{tabular}}
\end{table}
\end{comment}

\begin{table}[h!] 
\caption{A list of the free parameters entering the \textsc{emcee} algorithm in Runs M-A and A. The ``Nelder-Mead" column marks the parameters which were optimized before running \textsc{emcee}, in order to speed-up the convergence of the posterior distributions.} \label{tab4}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{l<{\raggedleft}m{7cm}|ccc}
\hline
\hline
\multirow{2}*{Parameter} & \multirow{2}*{Description} & Run M-A & \multicolumn{2}{c}{Run A}\\
&& \textsc{emcee} & Nelder-Mead & \textsc{emcee}\\
\hline
$e \cos{\omega}$ &  &  & \checkmark & \checkmark\\
$e \sin{\omega}$ &  &  & \checkmark & \checkmark\\
$f$ & Flux scaling factor & \checkmark &  &\\
$f_c$ & $\sqrt{e}\cos{\omega}$ & \checkmark &  &\\
$f_s$ & $\sqrt{e}\sin{\omega}$ & \checkmark &  &\\
$h_\text{1,F}, h_\text{2,F}$ & Parameters of the power-2 limb darkening law for star 1 & \checkmark &  & \\
$h_\text{1,K}, h_\text{2,K}$ & Parameters of the power-2 limb darkening law for star 2 & \checkmark &  & \\
$i$ & Orbital inclination & \checkmark & \checkmark & \checkmark\\
$k$ & Ratio of the radii & \checkmark &  &\\
$l_3$ & Third light & \checkmark &  & \checkmark\\
$L_\mathrm{pb}$ & Passband luminosity &  &  & \checkmark\\
$r_{sum}$ & Sum of the fractional radii & \checkmark &  &\\
$R_1$ & Radius of the primary star &  & \checkmark & \checkmark\\
$R_2$ & Radius of the secondary star &  & \checkmark & \checkmark\\
$\sigma_f$ & Standard error per observation & \checkmark &  &\\
$S_{\text{T}}$ & Surface brightness ratio averaged over the stellar disks in the TESS band & \checkmark &  &\\
$T_\text{0}$ & Time of primary eclipse & \checkmark & \checkmark & \checkmark\\
$T_\text{secondary}/T_\text{primary}$ & Ratio of the effective temperatures &  & \checkmark & \checkmark\\
\hline
\hline
\end{tabular}}
\end{table}

Despite the differences in the initial set-ups for the runs, we expected our results to agree with those obtained by \citet{maxted2020} within the reported uncertainties. However, Fig.~\ref{fig:comparison} shows that this is not the case as none of the results from Runs A–K lies in the 1-sigma spread of the \citet{maxted2020} values. As to the reason behind this discrepancy, multiple explanations present themselves. First, due to time and computational constraints, our \textsc{emcee} runs did not include nearly as many iterations as the runs in \citet{maxted2020}. Thus, there is a possibility that they might not have fully converged. %However, our runs yielded fairly consistent results, so this probably was not that big of an issue.
All of our runs, however, were treated consistently with each other, and still exhibit the influence of a number of decisions in the fitting process on the final results. Next, the mapping between the \textsc{PHOEBE} and \textsc{ellc} parameterizations includes several assumptions and approximations, which leads to residuals between the two forward models (see Fig.~\ref{fig:model_resids}). This suggests that the offset between the two sets of results might be caused by not employing the native \textsc{PHOEBE} backend.

%In practice, these residuals suggest that we might need to switch to the native PHOEBE forward model in order to complete the convergence, obtain the final parameter values together with their uncertainties, and reach agreement with the results presented in \citet{maxted2020}.

%Although it is possible that selection of free parameters and their initial distributions might have stronger effect on the final results than anticipated, it is far more likely that the disagreement is caused by an error in the (yet unreleased) version of the Python module \phoebe{} that we used for the execution of Runs A–K. Indeed, preliminary analysis already revealed possible problems with the calculation of the surface-brightness ratio and conversion of units within Message Passing Interface (MPI). Nevertheless, a more thorough investigation is certainly required to identify the underlying issues and resolve the observed discrepancy.



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{final/figures/flux_resid_ellc_phoebe.eps}
    \caption{Residuals between the \textsc{ellc} and PHOEBE forward models for the nominal case.  This shows the influence of the approximations in mapping between the parameterization of the different codes and likely explains the offset between the results from our controlled sample and those in \citet{maxted2020}.  }
    \label{fig:model_resids}
\end{figure}

==> 5_-_Conclusion.tex <==
\section{Conclusions}
\begin{comment}
In this work, we tried to fit the parameters of the AI Phoenicis from the \TESS{} light curve and to reproduce the values estimated by \cite{maxted2020}.
First, we independently modeled the light curves with individual sets of free parameters and their approximations, e.g., \textbf{some info here}. Since our independent models did not lead to the same results for the system parameters of AI Phe, we designed a controlled experiment to systematically analyze the effect of the parameterization of individual parameters.  
%So after the first attempt to recreate the parameters we switch to a controlled experiment of modeling runs to look at the influence of different fitting choices on the results. 

The parameters obtained from different runs were expected to be distributed in a parameter space as found in \cite{maxted2020} but we find our results to be quite different in comparison to the accuracy that has been found before. We saw hints about the reason for this discrepancy in the residuals between \textsc{ellc} ``wrapper" and the \textsc{PHOEBE} forward models. Also, the runs in \cite{maxted2020} had more iterations and we suspect that one of the reasons for the difference might be the lack of computational time for our fit of the models.
%The difference between the parameters of our controlled runs and runs from the article from  \cite{maxted2020} was small but our results and results from \cite{maxted2020} are grouped in two clusters.
%More investigation is required to identify the underlying issues.
Though we cannot reach the accuracy we were looking for, \phoebe{} is still a powerful tool in modeling EBs when used with its own backend. This keeps open the scope to improve the \phoebe{} wrappers around different models and meanwhile, test our controlled experiment using the native backend and more computational time.
\end{comment}
%\begin{comment}
%- Donat
In this work, we tried to fit the parameters of AI Phoenicis from the \TESS{} light curve and to reproduce the values estimated by \cite{maxted2020}.
First, we independently modeled the light curves with individual sets of free parameters and their approximations, e.g., difference between initialized parameters of binary masses, radius, effective temperatures of the stars, or model of limb darkening, reflections etc. Since our independent models did not lead to the same results for the system parameters of AI Phe, we designed a controlled experiment to systematically analyze the effect of the parameterization. 

The parameters obtained from different runs were expected to be distributed in a parameter space as found in \cite{maxted2020} but we find our results to be quite different in comparison to the accuracy that has been found before. We suspect the discrepancy may be reconciled by running \textsc{emcee} for substantially longer to allow further convergence and to switch to the native PHOEBE forward model to avoid the assumptions and approximations in the translation between parameterizations.  Our results do, however, show the importance of several different choices in the fitting process on the final parameter values and their uncertainties.

%\end{comment}
